Loss-Free Machine Unlearning

We present a machine unlearning approach that is both retraining- and label-free. Most existing machine unlearning approaches require a model to be fine-tuned to remove information while preserving performance. This is computationally expensive and necessitates the storage of the whole dataset for the lifetime of the model. Retraining-free approaches often utilise Fisher information, which is derived from the loss and requires labelled data which may not be available. Thus, we present an extension to the Selective Synaptic Dampening algorithm, substituting the diagonal of the Fisher information matrix for the gradient of the l2 norm of the model output to approximate sensitivity. We evaluate our method in a range of experiments using ResNet18 and Vision Transformer. Results show our label-free method is competitive with existing state-of-the-art approaches.

==> Removed_guide_parts.tex <==
\section{Submission of tiny papers to ICLR 2024}

\textbf{The most important formatting requirement of the Tiny Papers 
track is that the main text (including title and abstract) is 
no more than two pages in length.} Appendices and references do not count
towards the page limit, however overly-long appendices, e.g., more than 10 pages, are 
not recommended and may be grounds for rejection.

\subsection{Style}

Papers to be submitted to the ICLR 2024 Tiny Papers track must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.

\vspace{4cm}
\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\vspace{3cm}
\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgements}
Use unnumbered third level headings for the acknowledgements. All
acknowledgements, including those to funding agencies, go at the end of the paper.

\subsubsection*{URM Statement}
Please include this URM Statement section at the end of the paper but before the references before. In your anonymized submission, we recommend stating ``The authors acknowledge that at least one key author of this work meets the URM criteria of ICLR 2024 Tiny Papers Track.'' For the camera ready version, we ask authors to identify which author(s) meet the URM criteria, e.g., ``Author TFB meets the URM criteria of ICLR 2024 Tiny Papers Track.'' The authors are also welcome to come up with their own phrases to affirm meeting this criteria.

==> old_tables.tex <==

\begin{table}[]
\centering
\caption{Fullclass unlearning on Cifar100 (baby-sea), Cifar20 (ED-Veh2), and Face unlearning. Parameters: Cifar100 with 10,1 for both; Cifar20 both 5,1; Faces with 10,1 \\}
\fontsize{9pt}{10pt}\selectfont
\setlength{\tabcolsep}{2.2pt}
\begin{tabular}{ll|cccc|cccc}
                            &                   & \multicolumn{4}{c|}{ResNet18}                                                                                                                                                   & \multicolumn{4}{c}{Vision Transformer}                                                                                        \\ \hline
\multicolumn{1}{l|}{Class}  & metric            & \multicolumn{1}{c|}{baseline}       & \multicolumn{1}{c|}{retrain}                                   & \multicolumn{1}{c|}{LFSSD}      & SSD                                     & \multicolumn{1}{c|}{baseline}       & \multicolumn{1}{c|}{retrain}        & \multicolumn{1}{c|}{LFSSD}  & SSD                  \\ \hline
\multicolumn{1}{l|}{baby}   & $\mathcal{D}_{r}$ & \multicolumn{1}{c|}{76.38$\pm$0.00} & \multicolumn{1}{c|}{73.10$\pm$0.55}                            & \multicolumn{1}{c|}{75.80$\pm$0.00}     & \textbf{44.05$\pm$0.00}                         & \multicolumn{1}{c|}{88.93$\pm$0.00} & \multicolumn{1}{c|}{90.27$\pm$0.15} & \multicolumn{1}{c|}{88.12$\pm$0.00} & 88.59$\pm$0.00       \\
\multicolumn{1}{l|}{}       & $\mathcal{D}_{f}$ & \multicolumn{1}{c|}{72.48$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}                             & \multicolumn{1}{c|}{0.00$\pm$0.00}         & 0.00$\pm$0.00                           & \multicolumn{1}{c|}{90.19$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}  & \multicolumn{1}{c|}{0.00$\pm$0.00}     & 0.00$\pm$0.00        \\
\multicolumn{1}{l|}{}       & MIA               & \multicolumn{1}{c|}{92.60$\pm$0.00} & \multicolumn{1}{c|}{2.44$\pm$0.01}                             & \multicolumn{1}{c|}{0.00$\pm$0.00}       & 5.40$\pm$0.00                          & \multicolumn{1}{c|}{75.60$\pm$0.00} & \multicolumn{1}{c|}{21.53$\pm$0.03} & \multicolumn{1}{c|}{4.00$\pm$0.00}   & 0.60$\pm$0.00        \\ \hline
\multicolumn{1}{l|}{lamp}   & $\mathcal{D}_{r}$ & \multicolumn{1}{c|}{76.39$\pm$0.00} & \multicolumn{1}{c|}{72.89$\pm$0.34}                            & \multicolumn{1}{c|}{76.36$\pm$0.00}     & 76.08$\pm$0.00                          & \multicolumn{1}{c|}{88.84$\pm$0.00} & \multicolumn{1}{c|}{90.10$\pm$0.19} & \multicolumn{1}{c|}{89.03$\pm$0.00} & 89.06$\pm$0.00       \\
\multicolumn{1}{l|}{}       & $\mathcal{D}_{f}$ & \multicolumn{1}{c|}{70.49$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}                             & \multicolumn{1}{c|}{0.00$\pm$0.00}         & 0.00$\pm$0.00                           & \multicolumn{1}{c|}{97.22$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}  & \multicolumn{1}{c|}{0.00$\pm$0.00}     & \textbf{36.89$\pm$0.00}       \\
\multicolumn{1}{l|}{}       & MIA               & \multicolumn{1}{c|}{92.40$\pm$0.00} & \multicolumn{1}{c|}{0.32$\pm$0.00}                             & \multicolumn{1}{c|}{0.00$\pm$0.00}         & 0.20$\pm$0.00                           & \multicolumn{1}{c|}{95.60$\pm$0.00} & \multicolumn{1}{c|}{2.27$\pm$0.01}  & \multicolumn{1}{c|}{2.20$\pm$0.00}   & 0.40$\pm$0.00        \\ \hline
\multicolumn{1}{l|}{MR}     & $\mathcal{D}_{r}$ & \multicolumn{1}{c|}{76.28$\pm$0.00} & \multicolumn{1}{c|}{72.90$\pm$0.45}                            & \multicolumn{1}{c|}{76.28$\pm$0.00}     & 75.59$\pm$0.00                          & \multicolumn{1}{c|}{88.87$\pm$0.00} & \multicolumn{1}{c|}{90.02$\pm$0.22} & \multicolumn{1}{c|}{88.93$\pm$0.00} & 88.82$\pm$0.00       \\
\multicolumn{1}{l|}{}       & $\mathcal{D}_{f}$ & \multicolumn{1}{c|}{80.12$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}                             & \multicolumn{1}{c|}{0.00$\pm$0.00}         & 0.00$\pm$0.00                           & \multicolumn{1}{c|}{94.88$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}  & \multicolumn{1}{c|}{0.00$\pm$0.00}     & 0.00$\pm$0.00        \\
\multicolumn{1}{l|}{}       & MIA               & \multicolumn{1}{c|}{95.20$\pm$0.00} & \multicolumn{1}{c|}{0.22$\pm$0.00}                             & \multicolumn{1}{c|}{0.00$\pm$0.00}       & 0.20$\pm$0.00                           & \multicolumn{1}{c|}{92.80$\pm$0.00} & \multicolumn{1}{c|}{0.70$\pm$0.00}  & \multicolumn{1}{c|}{2.60$\pm$0.00}   & 3.80$\pm$0.00        \\ \hline
\multicolumn{1}{l|}{Rkt}    & $\mathcal{D}_{r}$ & \multicolumn{1}{c|}{76.27$\pm$0.00} & \multicolumn{1}{c|}{72.83$\pm$0.42}                            & \multicolumn{1}{c|}{75.67$\pm$0.00}     & 74.54$\pm$0.00                          & \multicolumn{1}{c|}{88.88$\pm$0.00} & \multicolumn{1}{c|}{90.07$\pm$0.09} & \multicolumn{1}{c|}{88.86$\pm$0.00} & 88.90$\pm$0.00       \\
\multicolumn{1}{l|}{}       & $\mathcal{D}_{f}$ & \multicolumn{1}{c|}{80.90$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}                             & \multicolumn{1}{c|}{0.00$\pm$0.00}         & 0.00$\pm$0.00                           & \multicolumn{1}{c|}{94.70$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}  & \multicolumn{1}{c|}{0.00$\pm$0.00}     & 0.00$\pm$0.00        \\
\multicolumn{1}{l|}{}       & MIA               & \multicolumn{1}{c|}{93.40$\pm$0.00} & \multicolumn{1}{c|}{1.04$\pm$0.00}                             & \multicolumn{1}{c|}{0.00$\pm$0.00}         & 2.20$\pm$0.00                           & \multicolumn{1}{c|}{94.40$\pm$0.00} & \multicolumn{1}{c|}{3.23$\pm$0.00}  & \multicolumn{1}{c|}{10.60$\pm$0.00}   & 1.80$\pm$0.00        \\ \hline
\multicolumn{1}{l|}{sea}    & $\mathcal{D}_{r}$ & \multicolumn{1}{c|}{76.23$\pm$0.00} & \multicolumn{1}{c|}{72.83$\pm$0.54}                            & \multicolumn{1}{c|}{75.43$\pm$0.00}     & 73.56$\pm$0.00                          & \multicolumn{1}{c|}{88.91$\pm$0.00} & \multicolumn{1}{c|}{90.27$\pm$0.21} & \multicolumn{1}{c|}{88.67$\pm$0.00} & 87.95$\pm$0.00       \\
\multicolumn{1}{l|}{}       & $\mathcal{D}_{f}$ & \multicolumn{1}{c|}{85.85$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}                             & \multicolumn{1}{c|}{0.00$\pm$0.00}         & 0.00$\pm$0.00                           & \multicolumn{1}{c|}{90.54$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}  & \multicolumn{1}{c|}{0.00$\pm$0.00}     & 0.00$\pm$0.00        \\
\multicolumn{1}{l|}{}       & MIA               & \multicolumn{1}{c|}{93.40$\pm$0.00} & \multicolumn{1}{c|}{5.84$\pm$0.02}                             & \multicolumn{1}{c|}{0.00$\pm$0.00}       & 0.60$\pm$0.00                           & \multicolumn{1}{c|}{80.40$\pm$0.00} & \multicolumn{1}{c|}{8.43$\pm$0.02}  & \multicolumn{1}{c|}{4.20$\pm$0.00}   & 3.20$\pm$0.00        \\ \hline \hline

\multicolumn{1}{l|}{ED}     & $\mathcal{D}_{r}$ & \multicolumn{1}{c|}{82.56$\pm$0.00} & \multicolumn{1}{c|}{82.13$\pm$0.23}                            & \multicolumn{1}{c|}{83.19$\pm$0.00}     & 83.15$\pm$0.00                          & \multicolumn{1}{c|}{95.73$\pm$0.00} & \multicolumn{1}{c|}{94.71$\pm$0.14} & \multicolumn{1}{c|}{95.84$\pm$0.00} & 95.82$\pm$0.00       \\
\multicolumn{1}{l|}{}       & $\mathcal{D}_{f}$ & \multicolumn{1}{c|}{82.26$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}                             & \multicolumn{1}{c|}{0.00$\pm$0.00}         & 1.76$\pm$0.00                           & \multicolumn{1}{c|}{95.03$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}  & \multicolumn{1}{c|}{0.68$\pm$0.00}     & \textbf{53.53$\pm$0.00}       \\
\multicolumn{1}{l|}{}       & MIA               & \multicolumn{1}{c|}{89.56$\pm$0.00} & \multicolumn{1}{c|}{8.91$\pm$0.01}                             & \multicolumn{1}{c|}{3.80$\pm$0.00}      & 4.16$\pm$0.00                           & \multicolumn{1}{c|}{91.60$\pm$0.00} & \multicolumn{1}{c|}{9.82$\pm$0.01}  & \multicolumn{1}{c|}{4.00$\pm$0.00}  & 1.32$\pm$0.00        \\ \hline
\multicolumn{1}{l|}{NS}     & $\mathcal{D}_{r}$ & \multicolumn{1}{c|}{82.10$\pm$0.00} & \multicolumn{1}{c|}{81.33$\pm$0.22}                            & \multicolumn{1}{c|}{82.44$\pm$0.00}     & 82.33$\pm$0.00                          & \multicolumn{1}{c|}{95.71$\pm$0.00} & \multicolumn{1}{c|}{94.79$\pm$0.11} & \multicolumn{1}{c|}{95.13$\pm$0.00} & 93.63$\pm$0.00       \\
\multicolumn{1}{l|}{}       & $\mathcal{D}_{f}$ & \multicolumn{1}{c|}{91.08$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}                             & \multicolumn{1}{c|}{0.00$\pm$0.00}         & 0.00$\pm$0.00                           & \multicolumn{1}{c|}{95.37$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}  & \multicolumn{1}{c|}{0.00$\pm$0.00}     & 0.00$\pm$0.00        \\
\multicolumn{1}{l|}{}       & MIA               & \multicolumn{1}{c|}{88.68$\pm$0.00} & \multicolumn{1}{c|}{3.77$\pm$0.01}                             & \multicolumn{1}{c|}{2.68$\pm$0.00}      & 3.28$\pm$0.00                           & \multicolumn{1}{c|}{85.04$\pm$0.00} & \multicolumn{1}{c|}{4.70$\pm$0.01}  & \multicolumn{1}{c|}{4.72$\pm$0.00}     & 1.88$\pm$0.00        \\ \hline
\multicolumn{1}{l|}{people} & $\mathcal{D}_{r}$ & \multicolumn{1}{c|}{82.11$\pm$0.00} & \multicolumn{1}{c|}{81.20$\pm$0.19}                            & \multicolumn{1}{c|}{82.08$\pm$0.00}     & 82.31$\pm$0.00                          & \multicolumn{1}{c|}{95.54$\pm$0.00} & \multicolumn{1}{c|}{94.54$\pm$0.14} & \multicolumn{1}{c|}{95.50$\pm$0.00} & 95.33$\pm$0.00       \\
\multicolumn{1}{l|}{}       & $\mathcal{D}_{f}$ & \multicolumn{1}{c|}{90.70$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}                             & \multicolumn{1}{c|}{0.00$\pm$0.00}         & 0.00$\pm$0.00                           & \multicolumn{1}{c|}{98.54$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}  & \multicolumn{1}{c|}{2.52$\pm$0.00}     & 0.00$\pm$0.00        \\
\multicolumn{1}{l|}{}       & MIA               & \multicolumn{1}{c|}{91.72$\pm$0.00} & \multicolumn{1}{c|}{1.36$\pm$0.00}                             & \multicolumn{1}{c|}{1.36$\pm$0.00}      & 1.12$\pm$0.00                           & \multicolumn{1}{c|}{89.48$\pm$0.00} & \multicolumn{1}{c|}{1.56$\pm$0.00}  & \multicolumn{1}{c|}{1.00$\pm$0.00}  & 1.20$\pm$0.00        \\ \hline
\multicolumn{1}{l|}{veg}    & $\mathcal{D}_{r}$ & \multicolumn{1}{c|}{82.31$\pm$0.00} & \multicolumn{1}{c|}{81.39$\pm$0.21}                            & \multicolumn{1}{c|}{82.47$\pm$0.00}     & 82.38$\pm$0.00                          & \multicolumn{1}{c|}{95.59$\pm$0.00} & \multicolumn{1}{c|}{94.54$\pm$0.21} & \multicolumn{1}{c|}{95.64$\pm$0.00} & 95.71$\pm$0.00       \\
\multicolumn{1}{l|}{}       & $\mathcal{D}_{f}$ & \multicolumn{1}{c|}{86.90$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}                             & \multicolumn{1}{c|}{0.00$\pm$0.00}         & 0.00$\pm$0.00                           & \multicolumn{1}{c|}{97.57$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}  & \multicolumn{1}{c|}{0.59$\pm$0.00}     & 0.00$\pm$0.00        \\
\multicolumn{1}{l|}{}       & MIA               & \multicolumn{1}{c|}{89.52$\pm$0.00} & \multicolumn{1}{c|}{9.74$\pm$0.01}                             & \multicolumn{1}{c|}{5.44$\pm$0.00}     & 16.96$\pm$0.00                          & \multicolumn{1}{c|}{91.32$\pm$0.00} & \multicolumn{1}{c|}{4.41$\pm$0.01}  & \multicolumn{1}{c|}{3.00$\pm$0.000}  & 1.88$\pm$0.00        \\ \hline
\multicolumn{1}{l|}{Veh2}   & $\mathcal{D}_{r}$ & \multicolumn{1}{c|}{82.69$\pm$0.00} & \multicolumn{1}{c|}{82.11$\pm$0.19}                            & \multicolumn{1}{c|}{82.72$\pm$0.00}     & 82.97$\pm$0.00                          & \multicolumn{1}{c|}{95.73$\pm$0.00} & \multicolumn{1}{c|}{94.85$\pm$0.13} & \multicolumn{1}{c|}{95.94$\pm$0.00} & 93.12$\pm$0.00       \\
\multicolumn{1}{l|}{}       & $\mathcal{D}_{f}$ & \multicolumn{1}{c|}{80.41$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}                             & \multicolumn{1}{c|}{0.00$\pm$0.00}         & 0.00$\pm$0.00                           & \multicolumn{1}{c|}{95.22$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00}  & \multicolumn{1}{c|}{0.00$\pm$0.00}     & 0.00$\pm$0.00        \\
\multicolumn{1}{l|}{}       & MIA               & \multicolumn{1}{c|}{82.56$\pm$0.00} & \multicolumn{1}{c|}{13.54$\pm$0.01}                            & \multicolumn{1}{c|}{3.92$\pm$0.00}      & 6.68$\pm$0.00                           & \multicolumn{1}{c|}{84.04$\pm$0.00} & \multicolumn{1}{c|}{22.96$\pm$0.03} & \multicolumn{1}{c|}{9.12$\pm$0.00}  & 7.04$\pm$0.00        \\ \hline  \hline

\multicolumn{1}{l|}{Faces}  & $\mathcal{D}_{r}$ & \multicolumn{1}{c|}{98.52$\pm$0.02} & \multicolumn{1}{c|}{100.00$\pm$0.00} & \multicolumn{1}{c|}{98.15$\pm$0.20} & 98.42$\pm$0.13                          &                                     &                                     &                            & \multicolumn{1}{l}{} \\
\multicolumn{1}{l|}{}       & $\mathcal{D}_{f}$ & \multicolumn{1}{c|}{97.84$\pm$1.99} & \multicolumn{1}{c|}{0.00$\pm$0.00} & \multicolumn{1}{c|}{0.00$\pm$0.00} & 0.00$\pm$0.00 &                                     &                                     &                            & \multicolumn{1}{l}{} \\
\multicolumn{1}{l|}{}       & MIA               & \multicolumn{1}{c|}{34.38$\pm$0.23} & \multicolumn{1}{c|}{0.00$\pm$0.00}  & \multicolumn{1}{c|}{0.38$\pm$0.58} & 1.11$\pm$0.01                           &                                     &                                     &                            & \multicolumn{1}{l}{} \\ \cline{1-6}
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{Subclass unlearning on Cifar20. Parameters: RN and ViT with 10 and 1 \\}
\fontsize{9pt}{10pt}\selectfont
\setlength{\tabcolsep}{2.2pt}
\begin{tabular}{ll|cccc|cccc}
                           &                   & \multicolumn{4}{c|}{ResNet18}                                                                                          & \multicolumn{4}{c}{Vision Transformer}                                                                                 \\ \hline
\multicolumn{1}{l|}{Class} & metric            & \multicolumn{1}{c|}{baseline}       & \multicolumn{1}{c|}{retrain}        & \multicolumn{1}{c|}{LFSSD} & SSD            & \multicolumn{1}{c|}{baseline}       & \multicolumn{1}{c|}{retrain}        & \multicolumn{1}{c|}{LFSSD} & SSD            \\ \hline
\multicolumn{1}{l|}{baby}  & $\mathcal{D}_{r}$ & \multicolumn{1}{c|}{82.45$\pm$0.00} & \multicolumn{1}{c|}{81.45$\pm$0.3}  & \multicolumn{1}{c|}{78.93$\pm$0.00}     & 79.25$\pm$0.00 & \multicolumn{1}{c|}{95.69$\pm$0.00} & \multicolumn{1}{c|}{94.50$\pm$0.19} & \multicolumn{1}{c|}{95.38$\pm$0.00}     & 95.54$\pm$0.00 \\
\multicolumn{1}{l|}{}      & $\mathcal{D}_{f}$ & \multicolumn{1}{c|}{86.98$\pm$0.00} & \multicolumn{1}{c|}{80.03$\pm$3.4}  & \multicolumn{1}{c|}{0.78$\pm$0.00}     & 8.85$\pm$0.00  & \multicolumn{1}{c|}{96.44$\pm$0.00} & \multicolumn{1}{c|}{93.23$\pm$1.09} & \multicolumn{1}{c|}{86.81$\pm$0.00}     & 94.10$\pm$0.00 \\
\multicolumn{1}{l|}{}      & MIA               & \multicolumn{1}{c|}{90.40$\pm$0.00} & \multicolumn{1}{c|}{44.82$\pm$0.02} & \multicolumn{1}{c|}{1.00$\pm$0.00}     & 1.40$\pm$0.00  & \multicolumn{1}{c|}{91.60$\pm$0.00} & \multicolumn{1}{c|}{77.37$\pm$0.03} & \multicolumn{1}{c|}{1.60$\pm$0.00}    & 77.20$\pm$0.00 \\ \hline
\multicolumn{1}{l|}{lamp}  & $\mathcal{D}_{r}$ & \multicolumn{1}{c|}{82.61$\pm$0.00} & \multicolumn{1}{c|}{81.81$\pm$0.19} & \multicolumn{1}{c|}{81.54$\pm$0.00}     & 79.58$\pm$0.00 & \multicolumn{1}{c|}{95.77$\pm$0.00} & \multicolumn{1}{c|}{94.69$\pm$0.13} & \multicolumn{1}{c|}{95.68$\pm$0.00}     & 95.54$\pm$0.00 \\
\multicolumn{1}{l|}{}      & $\mathcal{D}_{f}$ & \multicolumn{1}{c|}{72.66$\pm$0.00} & \multicolumn{1}{c|}{22.95$\pm$4.72} & \multicolumn{1}{c|}{7.29$\pm$0.00}     & 0.00$\pm$0.00  & \multicolumn{1}{c|}{89.58$\pm$0.00} & \multicolumn{1}{c|}{34.55$\pm$8.62} & \multicolumn{1}{c|}{24.05$\pm$0.00}     & 14.58$\pm$0.00 \\
\multicolumn{1}{l|}{}      & MIA               & \multicolumn{1}{c|}{83.40$\pm$0.00} & \multicolumn{1}{c|}{4.29$\pm$0.01}  & \multicolumn{1}{c|}{3.40$\pm$0.00}     & 2.00$\pm$0.00  & \multicolumn{1}{c|}{81.00$\pm$0.00} & \multicolumn{1}{c|}{5.60$\pm$0.02}  & \multicolumn{1}{c|}{5.80$\pm$0.00}     & 3.2$\pm$0.00   \\ \hline
\multicolumn{1}{l|}{MR}    & $\mathcal{D}_{r}$ & \multicolumn{1}{c|}{82.60$\pm$0.00} & \multicolumn{1}{c|}{81.66$\pm$0.21} & \multicolumn{1}{c|}{80.38$\pm$0.00}     & 80.05$\pm$0.00 & \multicolumn{1}{c|}{95.69$\pm$0.00} & \multicolumn{1}{c|}{94.60$\pm$0.13} & \multicolumn{1}{c|}{95.66$\pm$0.00}     & 95.51$\pm$0.00 \\
\multicolumn{1}{l|}{}      & $\mathcal{D}_{f}$ & \multicolumn{1}{c|}{72.22$\pm$0.00} & \multicolumn{1}{c|}{10.48$\pm$2.02} & \multicolumn{1}{c|}{0.78$\pm$0.00}     & 0.78$\pm$0.00  & \multicolumn{1}{c|}{97.05$\pm$0.00} & \multicolumn{1}{c|}{26.57$\pm$6.41} & \multicolumn{1}{c|}{31.42$\pm$0.00}     & 6.68$\pm$0.00  \\
\multicolumn{1}{l|}{}      & MIA               & \multicolumn{1}{c|}{86.80$\pm$0.00} & \multicolumn{1}{c|}{2.27$\pm$0.00}  & \multicolumn{1}{c|}{3.80$\pm$0.00}     & 4.00$\pm$0.00  & \multicolumn{1}{c|}{77.80$\pm$0.00} & \multicolumn{1}{c|}{2.34$\pm$0.01}  & \multicolumn{1}{c|}{0.80$\pm$0.00}     & 0.40$\pm$0.00  \\ \hline
\multicolumn{1}{l|}{Rkt}   & $\mathcal{D}_{r}$ & \multicolumn{1}{c|}{82.54$\pm$0.00} & \multicolumn{1}{c|}{81.54$\pm$0.24} & \multicolumn{1}{c|}{80.49$\pm$0.00}     & 82.43$\pm$0.00 & \multicolumn{1}{c|}{95.73$\pm$0.00} & \multicolumn{1}{c|}{94.61$\pm$0.13} & \multicolumn{1}{c|}{95.66$\pm$0.00}     & 95.13$\pm$0.00 \\
\multicolumn{1}{l|}{}      & $\mathcal{D}_{f}$ & \multicolumn{1}{c|}{79.34$\pm$0.00} & \multicolumn{1}{c|}{10.74$\pm$3.4}  & \multicolumn{1}{c|}{0.00$\pm$0.00}     & 2.17$\pm$0.00  & \multicolumn{1}{c|}{94.53$\pm$0.00} & \multicolumn{1}{c|}{22.26$\pm$8.34} & \multicolumn{1}{c|}{2.17$\pm$0.00}     & 5.12$\pm$0.00  \\
\multicolumn{1}{l|}{}      & MIA               & \multicolumn{1}{c|}{89.40$\pm$0.00} & \multicolumn{1}{c|}{3.85$\pm$0.01}  & \multicolumn{1}{c|}{6.60$\pm$0.00}     & 10.80$\pm$0.00 & \multicolumn{1}{c|}{80.40$\pm$0.00} & \multicolumn{1}{c|}{3.44$\pm$0.01}  & \multicolumn{1}{c|}{3.00$\pm$0.00}     & 5.40$\pm$0.00  \\ \hline
\multicolumn{1}{l|}{sea}   & $\mathcal{D}_{r}$ & \multicolumn{1}{c|}{82.37$\pm$0.00} & \multicolumn{1}{c|}{81.30$\pm$0.27} & \multicolumn{1}{c|}{79.84$\pm$0.00}     & 81.72$\pm$0.00 & \multicolumn{1}{c|}{95.67$\pm$0.00} & \multicolumn{1}{c|}{94.55$\pm$0.22} & \multicolumn{1}{c|}{94.45$\pm$0.00}     & 95.57$\pm$0.00 \\
\multicolumn{1}{l|}{}      & $\mathcal{D}_{f}$ & \multicolumn{1}{c|}{96.27$\pm$0.00} & \multicolumn{1}{c|}{91.47$\pm$1.92} & \multicolumn{1}{c|}{18.06$\pm$0.00}     & 75.35$\pm$0.00 & \multicolumn{1}{c|}{99.22$\pm$0.00} & \multicolumn{1}{c|}{95.12$\pm$0.81} & \multicolumn{1}{c|}{20.83$\pm$0.00}     & 97.05$\pm$0.00 \\
\multicolumn{1}{l|}{}      & MIA               & \multicolumn{1}{c|}{90.80$\pm$0.00} & \multicolumn{1}{c|}{52.09$\pm$0.03} & \multicolumn{1}{c|}{2.20$\pm$0.00}    & 21.80$\pm$0.00 & \multicolumn{1}{c|}{88.40$\pm$0.00} & \multicolumn{1}{c|}{65.96$\pm$0.04} & \multicolumn{1}{c|}{6.60$\pm$0.00}     & 82.20$\pm$0.00 \\ \hline
\end{tabular}
\end{table}



\begin{table}[]
\centering
\caption{Random unlearning on Cifar 10. Parameters: RN 3.5, 1; ViT 3.5; 1 \\}
\fontsize{9pt}{10pt}\selectfont
\setlength{\tabcolsep}{2.2pt}
\begin{tabular}{l|lccc|lccc}
                  & \multicolumn{4}{c|}{ResNet18}                                                                                                                                              & \multicolumn{4}{c}{Vision Transformer}                                                                                                                                                               \\ \hline
metric            & \multicolumn{1}{c|}{baseline}       & \multicolumn{1}{c|}{retrain}                                  & \multicolumn{1}{c|}{LFSSD} & SSD                                      & \multicolumn{1}{c|}{baseline}                                 & \multicolumn{1}{c|}{retrain}                                  & \multicolumn{1}{c|}{LFSSD} & SSD                                      \\ \hline
$\mathcal{D}_{r}$ & \multicolumn{1}{l|}{90.71$\pm$0.00} & \multicolumn{1}{c|}{91.45$\pm$0.11} & \multicolumn{1}{c|}{89.$\pm$2.30}     & 88.68$\pm$3.36                           & \multicolumn{1}{l|}{98.88$\pm$0.00} & \multicolumn{1}{c|}{98.61$\pm$0.08}                           & \multicolumn{1}{c|}{98.53$\pm$0.27}     & 98.01$\pm$1.56 \\
$\mathcal{D}_{f}$ & \multicolumn{1}{l|}{95.30$\pm$2.08} & \multicolumn{1}{c|}{94.10$\pm$2.00} & \multicolumn{1}{c|}{94.94$\pm$2.89}     & 93.61$\pm$4.99 & \multicolumn{1}{l|}{100.00$\pm$0.00}                          & \multicolumn{1}{c|}{98.80$\pm$0.76} & \multicolumn{1}{c|}{99.52$\pm$0.84}     & 98.07$\pm$2.35 \\
MIA               & \multicolumn{1}{l|}{75.78$\pm$0.04} & \multicolumn{1}{c|}{74.22$\pm$0.04} & \multicolumn{1}{c|}{73.86$\pm$6.33}     & 72.65$\pm$0.05 & \multicolumn{1}{l|}{90.76$\pm$0.03}                           & \multicolumn{1}{c|}{91.77$\pm$0.02} & \multicolumn{1}{c|}{90.12$\pm$3.40}     & 85.54$\pm$0.11 \\ \hline
\end{tabular}
\end{table}
